N-GCN: Multi-scale Graph Convolution for Semi-supervised Node Classification

Graph Convolutional Networks (GCNs) have shown significant improvements in semi-supervised learning on graph-structured data. Concurrently, unsupervised learning of graph embeddings has benefited from the information contained in random walks. In this paper, we propose a model: Network of GCNs (N-GCN), which marries these two lines of work. At its core, N-GCN trains multiple instances of GCNs over node pairs discovered at different distances in random walks, and learns a combination of the instance outputs which optimizes the classification objective. Our experiments show that our proposed N-GCN model improves state-of-the-art baselines on all of the challenging node classification tasks we consider: Cora, Citeseer, Pubmed, and PPI. In addition, our proposed method has other desirable properties, including generalization to recently proposed semi-supervised learning methods such as GraphSAGE, allowing us to propose N-SAGE, and resilience to adversarial input perturbations.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	sample-manuscript.tex \
	sample-acmsmall.tex \
	sample-acmlarge.tex \
	sample-acmtog.tex \
	sample-sigconf.tex \
	sample-sigconf-authordraft.tex \
	sample-sigplan.tex \
	sample-sigchi.tex \
	sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf sample-*.pdf *.cls


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

==> feature_removal_cora.tex <==
\begin{tabular}{rccccc|| c c c }
	& \multicolumn{5}{c||}{\textbf{Features Removed}} & \multicolumn{3}{c}{\textbf{Train Nodes per class}} \\
	&   10\%  & 30\%  & 50\%  & 70\%  & 90\% & 20 & 10 &  5 \\
	%& \makebox{ &  \\ 
	\\
	%\cline{1-6} &  \\
	\hline \\
	\textbf{GCN}  & $81.2$  & $79.5$  & $75.8$  & $70.9$  & $59.4$ & $81.4$ & $73.2$ & $61.2$ \\
	$\textrm{\textbf{NGCN}}_\textrm{a}$  & $81.5$  & $80.3$  & $78.3$  & $74.8$  & $69.1$ & $82.4$ & $73.3$ & $61.4$ \\
	$\textrm{\textbf{NGCN}}_\textrm{a}$ (calibrated)  & $\mathbf{81.8}$  & $\mathbf{80.4}$  & $\mathbf{78.8}$  & $\mathbf{75.4}$  & $\mathbf{70.6}$ & $\mathbf{82.8}$ & $\mathbf{74.0}$ & $\mathbf{64.8}$ \\
\end{tabular}

==> link_removal_cora.tex <==
\begin{tabular}{lccccccccc}
\textbf{Edges Removed}   & 10\%  & 30\%  & 50\%  & 70\%  & 90\%  \\
\hline \\
\textbf{GCN}  & $76.9 \pm 0.060$   & $71.3 \pm 0.012$   & $55.3 \pm 0.018$   & $30.2 \pm 0.034$   & $15.3 \pm 0.012$   \\
$\textrm{\textbf{NGCN}}_\textrm{a}\ [K=5]$  & $80.1 \pm 0.005$   & $71.8 \pm 0.008$   & $56.2 \pm 0.013$   & $31.1 \pm 0.021$   & $15.5 \pm 0.008$   \\
\end{tabular}


==> result_summary_table.tex <==
\begin{tabular}{lccc}
\textbf{Method}  & \textbf{Pubmed} & \textbf{Citeseer} & \textbf{Cora} \\ \hline \\
ManiReg \citep{manireg}& $70.7$ & $60.1$ & $59.5$ \\ 

SemiEmb \citep{semiemb}& $71.1$ & $59.6$ & $59.0$ \\ 

LP \citep{lp}& $63.0$ & $45.3$ & $68.0$ \\ 

DeepWalk \citep{deepwalk}& $65.3$ & $43.2$ & $67.2$ \\ 

ICA \citep{ica}& $73.9$ & $69.1$ & $75.1$ \\ 

Planetoid \citep{planetoid}& $77.2$ & $64.7$ & $75.7$ \\ 

GCN \citep{kipf}& $79.0$ & $70.3$ & $81.5$ \\ 

\hline \hline
GCN (our implementation)& $79.2 \pm 0.35$ & $71.5 \pm 0.70$ & $81.2 \pm 0.65$ \\ 

$\textrm{NGCN}_\textrm{a}$ (ours)& $79.5 \pm 0.30$ & $\mathbf{71.9 \pm 0.05}$ & $\mathbf{82.4 \pm 0.30}$ \\ 

$\textrm{NGCN}_\textrm{fc}$ (ours)& $\mathbf{79.8 \pm 0.80}$ & $71.4 \pm 0.35$ & $82.1 \pm 0.30$ \\ 

\hline \hline
$\textrm{NGCN}_\textrm{a}$ (ours, calibrated)& $79.6 \pm 0.20$ & $71.6 \pm 0.10$ & $82.8 \pm 0.20$ \\ 

$\textrm{NGCN}_\textrm{fc}$ (ours, calibrated)& $\mathbf{80.9 \pm 0.35}$ & $\mathbf{74.3 \pm 0.35}$ & $\mathbf{84.5 \pm 0.30}$ \\

\end{tabular}


==> sweep_tables.tex <==
\begin{table}[h]
\input{sweeps/citeseer_gcn_a_0.tex}
\caption{N-GCN$_\textrm{a}$ results on Citeseer dataset, with $\hat{A}^0$ disabled. Top-left entry corresponds to vanilla GCN. Left column corresponds to ensemble of GCN models.}
\end{table}
\begin{table}[h]
\input{sweeps/citeseer_gcn_a_1.tex}
\caption{N-GCN$_\textrm{a}$ results on Citeseer dataset, with $\hat{A}^0$ enabled.}
\end{table}
\begin{table}[h]
\input{sweeps/citeseer_gcn_fc_0.tex}
\caption{N-GCN$_\textrm{fc}$ results on Citeseer dataset, with $\hat{A}^0$ disabled. Left column corresponds to ensemble of GCN models.}
\end{table}
\begin{table}[h]
\input{sweeps/citeseer_gcn_fc_1.tex}
\caption{N-GCN$_\textrm{fc}$ results on Citeseer dataset, with $\hat{A}^0$ enabled.}
\end{table}
\begin{table}[h]
\input{sweeps/citeseer_sage_a_0.tex}
\caption{N-SAGE$_\textrm{a}$ results on Citeseer dataset, with $\hat{A}^0$ disabled. Top-left entry corresponds to vanilla SAGE. Left column corresponds to ensemble of SAGE models.}
\end{table}
\begin{table}[h]
\input{sweeps/citeseer_sage_a_1.tex}
\caption{N-SAGE$_\textrm{a}$ results on Citeseer dataset, with $\hat{A}^0$ enabled.}
\end{table}
\begin{table}[h]
\input{sweeps/citeseer_sage_fc_0.tex}
\caption{N-SAGE$_\textrm{fc}$ results on Citeseer dataset, with $\hat{A}^0$ disabled. Left column corresponds to ensemble of SAGE models.}
\end{table}
\begin{table}[h]
\input{sweeps/citeseer_sage_fc_1.tex}
\caption{N-SAGE$_\textrm{fc}$ results on Citeseer dataset, with $\hat{A}^0$ enabled.}
\end{table}
\begin{table}[h]
\input{sweeps/cora_gcn_a_0.tex}
\caption{N-GCN$_\textrm{a}$ results on Cora dataset, with $\hat{A}^0$ disabled. Top-left entry corresponds to vanilla GCN. Left column corresponds to ensemble of GCN models.}
\end{table}
\begin{table}[h]
\input{sweeps/cora_gcn_a_1.tex}
\caption{N-GCN$_\textrm{a}$ results on Cora dataset, with $\hat{A}^0$ enabled.}
\end{table}
\begin{table}[h]
\input{sweeps/cora_gcn_fc_0.tex}
\caption{N-GCN$_\textrm{fc}$ results on Cora dataset, with $\hat{A}^0$ disabled. Left column corresponds to ensemble of GCN models.}
\end{table}
\begin{table}[h]
\input{sweeps/cora_gcn_fc_1.tex}
\caption{N-GCN$_\textrm{fc}$ results on Cora dataset, with $\hat{A}^0$ enabled.}
\end{table}
\begin{table}[h]
\input{sweeps/cora_sage_a_0.tex}
\caption{N-SAGE$_\textrm{a}$ results on Cora dataset, with $\hat{A}^0$ disabled. Top-left entry corresponds to vanilla SAGE. Left column corresponds to ensemble of SAGE models.}
\end{table}
\begin{table}[h]
\input{sweeps/cora_sage_a_1.tex}
\caption{N-SAGE$_\textrm{a}$ results on Cora dataset, with $\hat{A}^0$ enabled.}
\end{table}
\begin{table}[h]
\input{sweeps/cora_sage_fc_0.tex}
\caption{N-SAGE$_\textrm{fc}$ results on Cora dataset, with $\hat{A}^0$ disabled. Left column corresponds to ensemble of SAGE models.}
\end{table}
\begin{table}[h]
\input{sweeps/cora_sage_fc_1.tex}
\caption{N-SAGE$_\textrm{fc}$ results on Cora dataset, with $\hat{A}^0$ enabled.}
\end{table}
\begin{table}[h]
\input{sweeps/pubmed_gcn_a_0.tex}
\caption{N-GCN$_\textrm{a}$ results on Pubmed dataset, with $\hat{A}^0$ disabled. Top-left entry corresponds to vanilla GCN. Left column corresponds to ensemble of GCN models.}
\end{table}
\begin{table}[h]
\input{sweeps/pubmed_gcn_a_1.tex}
\caption{N-GCN$_\textrm{a}$ results on Pubmed dataset, with $\hat{A}^0$ enabled.}
\end{table}
\begin{table}[h]
\input{sweeps/pubmed_gcn_fc_0.tex}
\caption{N-GCN$_\textrm{fc}$ results on Pubmed dataset, with $\hat{A}^0$ disabled. Left column corresponds to ensemble of GCN models.}
\end{table}
\begin{table}[h]
\input{sweeps/pubmed_gcn_fc_1.tex}
\caption{N-GCN$_\textrm{fc}$ results on Pubmed dataset, with $\hat{A}^0$ enabled.}
\end{table}
\begin{table}[h]
\input{sweeps/pubmed_sage_a_0.tex}
\caption{N-SAGE$_\textrm{a}$ results on Pubmed dataset, with $\hat{A}^0$ disabled. Top-left entry corresponds to vanilla SAGE. Left column corresponds to ensemble of SAGE models.}
\end{table}
\begin{table}[h]
\input{sweeps/pubmed_sage_a_1.tex}
\caption{N-SAGE$_\textrm{a}$ results on Pubmed dataset, with $\hat{A}^0$ enabled.}
\end{table}
\begin{table}[h]
\input{sweeps/pubmed_sage_fc_0.tex}
\caption{N-SAGE$_\textrm{fc}$ results on Pubmed dataset, with $\hat{A}^0$ disabled. Left column corresponds to ensemble of SAGE models.}
\end{table}
\begin{table}[h]
\input{sweeps/pubmed_sage_fc_1.tex}
\caption{N-SAGE$_\textrm{fc}$ results on Pubmed dataset, with $\hat{A}^0$ enabled.}
\end{table}

